Voltage Constrained Heavy Duty Vehicle Electrification: Formulation and Case Study

The electrification of heavy-duty vehicles (HDEVs) is a rapidly emerging avenue for decarbonization of energy and transportation sectors. Compared to light duty vehicles, HDEVs exhibit unique travel and charging patterns over long distances. In this paper, we formulate an analytically tractable model that considers the routing decisions for the HDEVs and their charging implications on the power grid. Our model captures the impacts of increased vehicle electrification on the transmission grid, with particular focus on HDEVs. We jointly model transportation and power networks coupling them through the demand generated for charging requirements of HDEVs. In particular, the voltage constraint violation is explicitly accounted for in the proposed model given the signifcant amount of charging power imposed by HDEVs. We obtain optimal routing schedules and generator dispatch satisfying mobility constraints of HDEVs while minimizing voltage violations in electric transmission network. Case study based on an IEEE 24-bus system is presented using realistic data of transit data of HDEVs. The numerical results suggest that the proposed model and algorithm effectively mitigate the voltage violation when a significant amount of HDEVs are integrated to the power transmission network. Such mitigation includes reduction in the voltage magnitude, geographical dispersion of voltage violations and worst-case voltage violations at critical nodes.

==> paper/case-study.tex <==
In this section, we adapt the results on scenario generation in dynamic environments~\cite{shukla2023scenario}. In the presence of market imperfections, the CNOs might choose to introduce mark-ups on their retail charging prices by posting a price different from (22) that exploits the customers’ lack of options by charging them more than the marginal cost. Imperfections can arise due to a geographic monopoly (based on absence of other CNOs in a certain region), high entry fees/sunk costs for CNOs, and customer switch- ing costs. In this case, the CNO’s daily objective will be dif- ferent from (31), also changing the resulting queue equilib- rium. Accordingly, the distributed welfare-maximizing whole- sale pricing mechanism proposed above would no longer be valid.
Studying dynamics of imperfect competition between CNOs and the resulting price distortions is a subject of future work. Instead, in this section, we assume a certain mark-up structure and discuss the effect of such price distortions on the ISO’s wholesale market price design problem. Assuming the CNOs’ retail pricing strategy still reflects wholesale price dynamics to a certain degree, the EV demand will be correlated with the wholesale price under a more complex structure. For example, suppose each CNO r chooses per unit electricity prices for its charging stations with the following mark-up structure com- pared to the wholesale price

\medskip 
Then, the resulting flow from the customers served by CNO r
under a noqueue pricing scheme can be described by the KKT conditions of the following side constrained flow optimization problem:
\medskip 
Hence,the wholesaleelectricity pricing problem can be thought of as a bilevel optimization problem. At the upper level, the ISO designs the electricity price and minimizes the cost of generation; while the lower- level problem characterizes the possible set of electricity loads that can be the result of a queue equilibrium under the specific retail pricing mechanism (34) adopted by the CNO. Using the notation defined in (20), the bilevel optimization problem can be cast as follows:

\medskip 
Under any mark-up structure, solving the above bilevel problem is nontrivial due to the nonconvexity in the objective function and the constraints. While the upper- and lower-level problems are convex individually, the nonconvexity arises as the optimiza- tion variables of the upper- and lower-level problems are coupled together through pt. Commonly, to solve such problems, one would replace the lower-level problem with its KKT conditions that describe the generalized queue equilibrium under price . Accordingly, (36) is known as a MPEC, which is NP-hard in general. We propose an efficient computational algorithm based on scenario generation along with tight guarantees for the non-convex optimization problem. 


==> paper/notation.tex <==
\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

%bold letters 
%math bold letters 
\def\mA{\mathbb{A}}
\def\mB{\mathbb{B}}
\def\mC{\mathbb{C}}
\def\mD{\mathbb{D}}
\def\mE{\mathbb{E}}
\def\mF{\mathbb{F}}
\def\mG{\mathbb{G}}
\def\mH{\mathbb{H}}
\def\mI{\mathbb{I}}
\def\mJ{\mathbb{J}}
\def\mK{\mathbb{K}}
\def\mL{\mathbb{L}}
\def\mM{\mathbb{M}}
\def\mN{\mathbb{N}}
\def\mO{\mathbb{O}}
\def\mP{\mathbb{P}}
\def\mQ{\mathbb{Q}}
\def\mR{\mathbb{R}}
\def\mS{\mathbb{S}}
\def\mT{\mathbb{T}}
\def\mU{\mathbb{U}}
\def\mV{\mathbb{V}}
\def\mW{\mathbb{W}}
\def\mX{\mathbb{X}}
\def\mY{\mathbb{Y}}
\def\mZ{\mathbb{Z}}

==> shared/packages.tex <==
\usepackage{natbib}
\usepackage{pifont}
\usepackage{verbatim}
\usepackage{todonotes}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{mathtools}
\usepackage{bbold}
\usepackage{thmtools} 
\usepackage{thm-restate}
\usepackage{enumerate}
\usepackage{graphicx}
\usepackage{float}
\usepackage{cancel}
\usepackage{geometry}
\usepackage{amsmath,amssymb, amsfonts}
\usepackage{color}
\usepackage[toc,page]{appendix}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\declaretheorem[name=Theorem,numberwithin=section]{thm}
%\declaretheorem[name=Lemma,numberwithin=section]{lem}
%\declaretheorem[name=Corollary,numberwithin=section]{cor}
%\declaretheorem[name=Proposition,numberwithin=section]{prop}

\bibliographystyle{apalike}
\usepackage{fullpage}
\usepackage{picture,bm}
\usepackage{xcolor}
\usepackage{url}
\usepackage[colorlinks=true,linkcolor=blue,citecolor=black,pagebackref=true]{hyperref}  
